Towards a certified reference monitor of the Android 10 permission system

Android is a platform for mobile devices that captures more than 85% of the total market-share. Currently, mobile devices allow people to develop multiple tasks in different areas. Regrettably, the benefits of using mobile devices are counteracted by increasing security risks. The important and critical role of these systems makes them a prime target for formal verification. In our previous work (LNCS 10855, https://doi.org/10.1007/978-3-319-94460-9_16), we exhibited a formal specification of an idealized formulation of the permission model of version \texttt{6} of Android. In this paper we present an enhanced version of the model in the proof-assistant Coq, including the most relevant changes concerning the permission system introduced on versions Nougat, Oreo, Pie and 10. The properties that we had proved earlier for the security model has been either revalidated or refuted, and new ones have been formulated and proved. Additionally, we make observations on the security of the most recent versions of Android. Using the programming language of Coq we have developed a functional implementation of a reference validation mechanism and certified its correctness. The formal development is about 23k LOC of Coq, including proofs.

==> application_figure.tex <==
\small
\begin{displaymath}
\begin{array}[t]{l@{\,}l@{\,\,}ll}
%\Activity\; , \Service\; , \BroadReceiv & ::= & \CompId & \it{Activities,\ services\ and\ broadcast\ receivers} \\ 
\ContProv & ::= & \CompId \times \Uri \to \Res & \\
&& \it{Content\ provider} \\ [1ex]
\Comp & ::= & \Activity\; | \; \Service\; | \; \BroadReceiv\; | \; \ContProv &  \\
&& \it{Application\ component} \\ [1ex]
\Comps & ::= & \setof{\Comp} & \\ 
&& \it{Set\ of\ components} \\[1ex]
\PermLvl & ::= & dangerous\; | \; normal\; |  \; signature \; | \; signature/system & \\
&& \it{Permission\ level} \\ [1ex]
%\PermLvl & ::= & \Dangerous\; | \Normal\; |  \Signature \; | \SignatureSystem & \text{Permission level} \\
\Perm & ::= & \PermId \times \PermLvl & \\
&& \it{Permission} \\ [1ex]
\Perms & ::= & \setof{\Perm} & \\
&& \it{Set\ of\ permissions} \\[1ex]
\OptionPerm & ::= & \ap{Some}{p} \; | \; none & \\
&& \it{A\ possible\ empty\ permission} \\[1ex] 
\CompPerms & ::= & \Comp \to \Perms & \\
&& \it{Components\ permissions} \\ [1ex]
\ContProvPerms & ::= & \ContProv \to \Perms & \\
&& \it{Content\ providers\ permissions} \\[1ex]
\ExtPerms & ::= & \OptionPerm \times \CompPerms \times \ContProvPerms \times \ContProvPerms & \\
&& \it{External\ permissions} \\ [1ex]
\UriPerms & ::= & \ContProv \to \Perms & \\
&& \it{URI\ permissions} \\[1ex]
\DelPerms & ::= & \ContProvs \times \UriPerms & \\
&& \it{Delegated\ permissions} \\ [1ex]
\Manifest & ::= & \ManifestTy &\\  
&& \it{Manifest} \\ [1ex]
\AppRes & ::= & \setof{\Res} & \\
&& \it{Application\ resources} \\[2ex] 
\App & ::= & \AppTy & \\
&& \it{Application} \\
\end{array}
\end{displaymath}


==> defs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% New commands
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%

\newcommand{\Coq}{\textsf{Coq}\xspace}
\newcommand{\CompCert}{\textsf{CompCert}\xspace}
\newcommand{\VirtualCert}{\textsf{VirtualCert}\xspace}


%Notation
%
\newcommand{\eqdef}{\stackrel{{\rm def}}{=}}
\newcommand{\snoc}{\mathbin{\raise 0.5ex\hbox{$\smallfrown$}}}
\newcommand{\cat}{\mathbin{\hbox{$\oplus$}}}
\newcommand{\hooklongrightarrow}{\lhook\joinrel\longrightarrow}
\newcommand{\step}[1]{%
	\mathbin{\lower0.55ex\hbox{$\lhook\joinrel\xrightarrow{#1}$}}}
\newcommand{\stepos}[2]{%
	\mathbin{\lower0.55ex\hbox{$\lhook\joinrel\xrightarrow[#2]{#1}$}}}
\newcommand{\steprel}[3]{\mbox{$#1\ \step{#2} #3$}}
\newcommand{\exttrace}[3]{(\steprel{#1}{#2}{#3})}
\newcommand{\sstep}{\mbox{$\hookrightarrow$}}
\newcommand{\con}{\overline}
\newcommand{\streamof}[1]{\mbox{$[#1]_{\infty}$}}
\newcommand{\cons}{::}
\newcommand{\strcons}[2]{\mbox{$#1 \cons #2$}}
\newcommand{\trace}[1]{\mbox{$trace(#1)$}}
\newcommand{\run}[1]{\mbox{$run(#1)$}}
\newcommand{\osaction}[1]{\mbox{\texttt{#1}}}
\newcommand{\sostep}{\mbox{$\rightarrowtail$}}
\newcommand{\ostep}[2]{%
          \mathbin{\lower0.55ex\hbox{$\lhook\joinrel\xrightarrow{#1,#2}$}}}
\newcommand{\exttraceleak}[4]{({#1}\ostep{#2}{#3}{#4})}

%
\newcommand{\salways}{\mbox{$\Box$}}
\newcommand{\always}[2]{\mbox{$\salways(#1 ,#2)$}}
\newcommand{\alwaysrel}[3]{\mbox{$\salways(#1 ,#2,#3)$}}
%
\newcommand{\seventually}{\mbox{$\Diamond$}}
\newcommand{\eventually}[2]{\mbox{$\seventually(#1 ,#2)$}}

\newcommand{\safe}[1]{\mbox{$Safe(#1)$}}
\newcommand{\lift}[1]{\mbox{$Lift(#1)$}}
%
\newcommand{\initstate}[1]{\mbox{$\ap{initial\_state}{#1}$}}

%
%references
%
\newcommand{\chapref}[1]{Chapter~\ref{#1}}
\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\ssecref}[1]{Subsection~\ref{#1}}
\newcommand{\thmref}[1]{Theorem~\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}
\newcommand{\defref}[1]{Definition~\ref{#1}}
\newcommand{\propref}[1]{Proposition~\ref{#1}}
\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\tableref}[1]{Table~\ref{#1}}
%
% Inference Rules (inductive)
%
\newcommand{\rulezero}[1]{\infer{{#1}}{\mbox{}}}
\newcommand{\ruleone}[2]{\infer{{#1}}{{#2}}}
\newcommand{\ruletwo}[3]{\infer{#1}{{#2}&{#3}}}
\newcommand{\rulethree}[4]{\infer{#1}{{#2}&{#3}&{#4}}}
%
% Inference Rules (co-inductive)
%
\newcommand{\rulezeroco}[1]{\infer={{#1}}{\mbox{}}}
\newcommand{\ruleoneco}[2]{\infer={{#1}}{{#2}}}
\newcommand{\ruletwoco}[3]{\infer={#1}{{#2}&{#3}}}
\newcommand{\rulethreeco}[4]{\infer={#1}{{#2}&{#3}&{#4}}}


% example of rule with side condition
\newcommand{\rulethrees}[5]{\infer[\tiny #1]{#2}{{#3}&{#4}&{#5}}}
\newcommand{\rulefour}[5]{\infer{#1}{{#2}&{#3}&{#4}&{#5}}}
%
%Records
%
%\newcommand{\labl}[1]{\mbox{$\sf{#1}$}}
\newcommand{\labl}[1]{\mbox{$#1$}}
\newcommand{\proj}[2]{\mbox{$#1.\labl{#2}$}} %projection. Record first,then label
% record symbols
\newcommand{\recl}{\mbox{${\bf \langle}$}}
\newcommand{\recr}{\mbox{${\bf \rangle}$}}
% record types and objects of arity up to 3 (non indented)
\newcommand{\reci}[2]{\mbox{$\recl\sub{\labl{#1}}{1}:#2\recr$}}
\newcommand{\recil}[2]{\mbox{$\recl#1:#2\recr$}}
\newcommand{\recii}[4]{\mbox{$\recl\labl{#1}: #2,\labl{#3}: #4\recr$}}
\newcommand{\reciil}[4]{\mbox{$\recl#1: #2,#3: #4\recr$}}
\newcommand{\reciii}[6]{\mbox{$\recl\labl{#1}:#2,\labl{#3}:#4,\labl{#5}:#6\recr$}}
\newcommand{\robi}[2]{\mbox{$\recl\labl{#1} = #2\recr$}}
\newcommand{\robil}[2]{\mbox{$\recl#1=#2\recr$}}
\newcommand{\robii}[4]{\mbox{$\recl\labl{#1} = #2,\labl{#3} = #4\recr$}}
\newcommand{\robiil}[4]{\mbox{$\recl#1 = #2,#3 = #4\recr$}}
\newcommand{\robiii}[6]{\mbox{$\recl\labl{#1} = #2,\labl{#3} = #4,\labl{#5} = #6\recr$}}
%generic record types and objects
\newcommand{\nrec}[3]{\mbox{$\recl\ \labl{#1}_{1}:\ {#2}_{1},\ldots\ ,\labl{#1}_{#3} :\ {#2}_{#3}\recr$}}
\newcommand{\nrecl}[3]{\mbox{$\recl\sub{#1}{1}:\sub{#2}{1},\ldots,\sub{#1}{#3}:\sub{#2}{#3}\recr$}}
\newcommand{\mrobj}[3]{\mbox{$\recl\sub{\labl{#1}}{1}=\sub{#2}{1},\ldots,\sub{\labl{#1}}{#3}=\sub{#2}{#3}\recr$}}
\newcommand{\mrobjl}[3]{\mbox{$\recl\sub{#1}{1}=\sub{#2}{1},\ldots,\sub{#1}{#3}=\sub{#2}{#3}\recr$}}
%
% Functions
%
\newcommand{\funtype}[2]{\mbox{$#1\ {\rightarrow}\ #2$}}
\newcommand{\ap}[2]{\mbox{$#1(#2)$}}
\newcommand{\bap}[3]{\mbox{$#1(#2,#3)$}}
\newcommand{\tap}[4]{\mbox{$#1(#2,#3,#4)$}}
\newcommand{\eqobj}[2]{\mbox{$#1\ =\ #2$}}
%
% Products
%
\newcommand{\prodtype}[2]{\mbox{$#1\ {\times}\ #2$}}
\newcommand{\pair}[2]{\mbox{$(#1,#2)$}}
%%
% Declarations
%
\newcommand{\obdecl}[2]{\mbox{$#1 : #2$}} %object of type
\newcommand{\eqdecl}[2]{\mbox{$#1\ \eqdef\ #2$}} %definitional equality
%
% Logic
%
\newcommand{\myforall}[3]{\mbox{$\forall\ #1 : #2 , #3$}} %(var,type,prop)
\newcommand{\myexists}[3]{\mbox{$\exists\ #1 : #2,\ #3$}} %(var,type,prop)
\newcommand{\mylet}[3]{\mbox{$\mathsf{let}\ (#1 : #2 = \
 #3)~\mathsf{in}$}} %(var,type,prop)
\newcommand{\vartype}[2]{(#1 : #2)}

\newcommand{\myimply}[2]{\mbox{$#1 \rightarrow #2$}}
\newcommand{\myand}[2]{\mbox{$#1\ \land\ #2$}}
\newcommand{\myor}[2]{\mbox{$#1\ \lor\ #2$}}

%State components equivalences
\newcommand{\eqv}[3]{\mbox{$#1{\sim}_{\!\!#2}#3$}}
\newcommand{\sub}[2]{\mbox{$#1_{\scriptsize #2}$}}
%\newcommand{\equpstcmp}[1]{\sub{\sim}{#1}}
%\newcommand{\equpstcmpA}[4]{\mbox{$#1\ \equpstcmp{#3\ =\ #4}\ #2$}}
\newcommand{\equpstcmpA}[3]{\mbox{$#2\ = #1.[#3]$}}
\newcommand{\equpstmapidx}[2]{\sub{\sim}{#1,#2}}
\newcommand{\equpstmapidxA}[4]{\mbox{$#1\ \equpstmapidx{#3}{#4}\ #2$}}
%
% maps
%
\newcommand{\mymap}[2]{\mbox{$#1\ \mapsto\ #2$}}
\newcommand{\mybmap}[3]{\mbox{$#1\ \mapsto_{#3}\ #2$}}

\newcommand{\mapap}[2]{\mbox{$#1[#2]$}}
\newcommand{\mapupd}[3]{\mbox{$#1[#2:=#3]$}}
%
%Inductive type
%
\newcommand{\indtypen}{\mbox{$I\ \eqdef\ c_1 : T_1\ |\,\ldots\ |\ c_n : T_n$}}
\newcommand{\indtypeii}[5]{\mbox{$#1\ \eqdef\ #2 : #3\ |\ #4 : #5$}}
\newcommand{\indtypeiii}[7]{\mbox{$#1\ \eqdef\ #2 : #3\ |\ #4 : #5\ |\ #6 :
#7$}}
%
%Lists
\newcommand{\emptylist}{\mbox{$\{\}$}}
%
%The attacker
\newcommand{\attacker}[1]{\mbox{$\cal{#1}$}}
%%%%%%%%%%%%%%%%%%%%%%%%%
%% Stealth
%%%%%%%%%%%%%%%%%%%%%%%%%
%Programs
\newcommand{\prog}[3]{\mbox{$\recl #1,#2,#3 \recr$}}
\newcommand{\assigninstr}[2]{\mbox{$#1 := #2$}}
\newcommand{\ifinstr}[2]{\mbox{${\tt if}\; #1\; #2$}}
\newcommand{\gotoinstr}[1]{\mbox{${\tt goto}\; #1$}}
\newcommand{\execinstr}{\mbox{$\leadsto$}}
\newcommand{\progstate}[2]{\mbox{$\recl #1, #2 \recr$}}
\newcommand{\stealthstate}[3]{\mbox{$\recl #1, #2, #3 \recr$}}
\newcommand{\stealthstep}{\mbox{$\rightharpoonup$}}
\newcommand{\judgestealth}[4]{\mbox{$#1\; \vdash\  #2 ; #3\; \stealthstep\ #4$}}
\newcommand{\instroflabel}[2]{\mbox{$\ap{#1}{n} = #2$}}
\newcommand{\instrstep}[5]{\mbox{$\recl #1, #2 \recr\ \execinstr\  \recl #3 , #4 \recr ; #5$}}
\newcommand{\progexec}{\mbox{$\Rightarrow$}}
\newcommand{\strapp}[2]{\mbox{$#1 :: #2$}}
\newcommand{\progexecrel}[3]{\mbox{$\recl #1, #2 \recr\ \progexec\  #3$}}
\newcommand{\transform}[1]{\mbox{$\overline{#1}$}}
\newcommand{\samenonstealths}[2]{\mbox{$#1 \equiv #2$}}
\newcommand{\stealths}[1]{\mbox{${\cal{stealths}}\;#1$}}
\newcommand{\vareq}[1]{\sub{\simeq}{#1}}
\newcommand{\pointlowvareq}[5]{\mbox{$#1\ \vareq{#3\;#4\;#5}\ #2$}}
\newcommand{\vareqweak}[1]{\sub{\sim}{#1}}
\newcommand{\lowvareqweak}[5]{\mbox{$#1\ \vareqweak{#3\;#4\;#5}\ #2$}}







==> installSemantic.tex <==
\cnote{corregirla, adecuar notación, uso de operaciones auxiliares (tienen que estar explicadas o referidas adecuadamente cuando se explica la poscondición, equivalencia de estados (no usar state+environment}


\begin{actdefrule}
\inferrule
{
{\begin{tabularx}{\linewidth}{X}
\begin{math}
\neg isAppInstalled(app,s)\ \land
\end{math}
\\
\begin{math}
\neg has\_duplicates\_cmp(m)\ \land
\end{math}
\\
\begin{math}
\forall c:\Comp, c \in cmp(m)\ \rightarrow\  c \notin cmpInState(s)\ \land
\end{math}
\\
\begin{math}
\neg hasDuplicates\_perm(m)\  \land
\end{math}
\\
\begin{math}
authPerms(m,s)\ \land
\end{math}
\\
\begin{math}
\forall c:\Comp, c \in cmp(m)\ \rightarrow\ cmpDeclareIntentFilterCorrectly(c)\ 
\end{math}
\\
\cnote{REVISAR:}\\
\begin{math}
addManifest(m,app,s,s')\land
\end{math}
\\
\begin{math}
addCert(c,app,s,s')\land
\end{math}
\\
\begin{math}
addDefPerms(app,m,s,s')\land
\end{math}
\\
\begin{math}
addApp(app,s,s')\land
\end{math}
\\
\begin{math}
addRes(app,lRes,s,s')\land
\end{math}
\\
\begin{math}
initializePermLists(app,s,s')\land
\end{math}
\\
\begin{math}
sameOtherFields\_install(s,s')\
%s.state \equiv_{running, delPPerms, delTPerms, sentIntents} s'.state
\end{math}
%\\
%\begin{math}
%s.environment \equiv_{systemImage} s'.environment
%\end{math}
%\\
\end{tabularx}}
}
{s \semstep{\ainstall{a~}{m~}{c~}{lRes}} s'}
\end{actdefrule}


==> monitor.tex <==
\section{Monitor error detection}
\label{sec:monitor}

An implementation of Android's security system, whose correction in regard of the model has been formally proved, may be used to compare the results of executing an action on an analyzed platform and executing that same action on the correct program. 
This gives us the possibility of developing a program capable monitoring the actions performed in a real system and evaluating if certain interesting properties hold on it, counting on the certified implementation to make comparisons.

Such monitor would be running alonside the platform under control, as a passive hypervisor. It must be able at any given time to intepret the system's state and constructing an equivalent state in the developed model. This operation will be called ``extracting'' the real state, and we will trust that it has been correctly developed; since this is the way of extrapolating the information stored in the real platform to a record of type $\AndroidState$ in \texttt{Coq} with which computations will be carried out.
%\fgnote{Aca había código C como ejemplo de una aplicacion real que no creo que valga la pena poner, ¿o sí? \\}
%\cnote{Si te parece que no aporta, no lo incluyas.\\}
Apart from the extraction of the platform state, the monitor must be aware of the internal representation, in the supervised implementation, of the modelled error codes. 
Finally, the monitor must have the power of intercepting the system calls able to mutate the certified implementation's state, and replicate them on it.
The activity of the monitor is depicted in Figure~\ref{fig:monitor:steps}, and consists of, when it detects the call to a function that represents the execution of a modeled action (2), extracting the state prior to its execution (1), replicating the performed action on it (3), extracting the state and the error code reached after the operation in the real platform (4), and finally compare them with the results obtained by the execution of the action in the extracted state (5). 

\begin{figure}[!htb]
\centering
\includegraphics[scale=0.55]{img/monitor_steps.png}
\caption{Monitor's activty.}
\label{fig:monitor:steps}
\end{figure}

These steps can be executed successively along the system's lifecycle, resulting in a program that monitors the truth of interesting properties in real time. 
Which properties to check and what to do when they don't hold is up to the monitor's configurator. 
For example, given a function $valid\_state\_bool : \AndroidState \to bool$ such that $\forall s, valid\_state(s) \iff valid\_state\_bool(s) = true$, it is feasible to develop a monitor that checks on runtime if the successive states a device goes through are valid; and act consequently in case they are not.
%\cnote{incluir los (tres) casos de uso.}

Nevertheless, the certified implementation developed is just one of all the possible correct implementations: a different result on a real platform doesn't necessarily imply a specification violation. 
Such a situation can be witnessed, for instance, in the $\texttt{install}~app~m~c~lRes$ action; its specification requires ---among other things--- that if its precondition is met, then $app$ is part of the list of installed applications in the reached state $s'$. The certified implementation prepends $app$ to the list of installed applications, but a system that chooses to append it to the end instead, is equally correct. To bypass this problem, the monitor's user may define an equivalence function between two systems and results gotten after performing the same action on the same initial state: 
$eq\_res : \Action \to \AndroidState \to Result \to Result \to bool$
which will be noted $\sim$, and we will say that given two results $r_1$ and $r_2$, an action $a$ and a state $s$,
$r_1 \underset{a,s}{\sim} r_2 \iff eq\_res~a~s~r1~r2=true$.
The idea behind the equivalence function is to allow the reuse of the proof of $step$'s soundness, by adjusting the technical differences between the certified implementation and the real platform that arise from the specification's non-determinism.
Naturally, the more these two diverge, the less can be reused from the original proof, and the effort invested in coding the equivalence function will be greater.


==> properties.tex <==
\newtheorem{prop}{Property}

\section{Security properties}
\label{sec:properties}
We have already extended the (formal) model presented in \cite{BetarteCLR16} so as to consider, in particular, the run time requesting/granting of permissions behavior introduced in Android Marshmallow. Also, we consider here executions that contemplate error management and a certified monitor of the security model.

In this section we present and discuss some relevant properties that can be established concerning the Android Marshmallow security framework.  
The helper functions and predicates used to define the lemmas discussed in this section are presented and described in Table \ref{tab:model:semantic_descriptions}. 
The full formal definition of the lemmas can be found in \cite{AndroidCoq:2016}, along with their proofs.
Likewise, in \cite{AndroidCoq:2016} other security properties are formally analyzed, which we omit here for reasons of space.

%\cnote{INCLUIR PROPIEDADES DE EJECUCIONES Y TRAZAS DE LA TESINA DE FELIPE\\}
%\fgnote{Solo ejecuciones y trazas? Todas ellas? \\ }
%\cnote{SI. Por una lado están las propiedades de seguridad del modelo(2.10 del informe) y tro lado están las propiedades sobre  trazas (3.5 del informe). Considero que hay que ponerlas a todas, agrupándolas en ds categorías (como en la tesina). Si en el paper tenemos luego que podar, nos quedan para una versión extendida (eventual journal).\\}

\input{auxfuns}

%We have stated and proved several security properties over the relation $\step{}$, showing that they hold on every correct implementation. \\

Lemma~\ref{modelproperty1} presents a controversial characteristic of Android's new permission system. For example, as the dangerous permissions $\mathsf{READ\_CONTACTS}$ (required for reading the contact list) and $\mathsf{WRITE\_CONTACTS}$ (required for writing the contact list) both belong the permission group $\mathsf{CONTACTS}$, none of them can be individually granted. Instead, the application must be granted the permission group $\mathsf{CONTACTS}$, giving it the right to both reading and writing the user's contact list. \\
The formal proof of this weak point should raise awareness of it during the specification of future versions of Android's permission system.

\begin{lemma} [noGranularityForIndividualPerms] \label{modelproperty1} \\
$\forall (s,s': \AndroidState) (p:\Perm) (g:\PermGrp) (app:\AppId),$ \\
$permissionIsGrouped(p) \rightarrow\ \neg \Mathexecrel{s}{\texttt{grant}~p~app/ok}{s'}$ \\ \\
\textit{Android's permission system isn't granular enough for granting a proper subset of the set of permissions that belong to a group.}\\
\end{lemma}


Lemma~\ref{modelproperty2} complements Lemma~\ref{modelproperty1}, and formalizes another weak point in the specification of Android's new permission system. Following the previous example, in a valid state an application may have the right of writing the contact list ($\mathsf{READ\_CONTACTS}$) even though this permission was never individually granted (since the application may have been granted the whole permission group $\mathsf{CONTACTS}$). \\
In a similar way as in lemma~\ref{modelproperty1}, the knowledge and formal description of this weak point should influence the roadmap of the evolution of the permission system.

\begin{lemma} [hasPermissionAndNotGranted] \label{modelproperty2}\\ 
$\exists (s:\AndroidState) (p:\Perm) (app:\AppId),$ % (permsA :\{Perm\}),$ \\
$valid\_state(s)\ \land \\
getPermissionLevel(p) = dangerous~ \land$ $p \notin getGrantedPermsForApp(app,s)~ \land$  \\ $p \notin getDefPermsForApp(app,s) \land appHasPermission(app,p,s)$ \\ \\
\textit{In contrast to what happened in previous Andorid versions, an application to which certain permission was never granted, may still have it.}\\
\end{lemma}

%\cnote{Revisar el siguiente lema: el enunciado (completamente), los elementos auxiliares no definidos, la cuantificación %sobre condiciones, la explicación...\\
In Android 6.0, an application that wishes to send information through the network must have the permission $\mathsf{INTERNET}$ but, since this permission is of level $normal$, any application that lists it as used in its manifest file has the right to access the network in an implicit and irrevocable way. Once again, this has been criticized due to the potential information leakage it allows. The following lemma formally generalizes this situation and embodies a reasonable argument to roll back this security issue introduced in Android Marshmallow. \\


\begin{lemma}[sacProtectedWithNormalPerms]\\
$ \forall (s:\AndroidState) (sac:SACall) (c:\Comp) (ic:\iComp) (p:\Perm), \\
valid\_state(s) \rightarrow permSAC(p, sac) \rightarrow \\
getPermissionLevel(p) = normal \rightarrow getPermissionId(p) \in \\
getAppRequestedPerms(getManifestForApp(getAppFromCmp(c,s),s)) \rightarrow\\
(ic, c) \in getRunningComponents(s) \rightarrow \Mathexecrel{s}{\texttt{call}~ic~sac/ok}{s}$ \\ \\
\textit{If the execution of an Android API call only requires permissions of level $normal$, it is enough for an application to list them as used on its manifest file to be allowed to perform such call.}\\
\end{lemma}


We have defined a function that allows the reference monitor to chain a list of actions processing them in order, whose definition is shown in \figref{fig:trace}.
\begin{figure}[ht]
\begin{displaymath}
\begin{array}{l}
	\textbf{Function}\ trace\ (s:\AndroidState)\ (actions:list\ \Action)\ :\ list\ \AndroidState \ := \\
	\quad \textbf{match}\ actions\ \textbf{with} \\
	\quad \hspace{1cm} |\ nil\ \Rightarrow\ nil \\
	\quad \hspace{1cm} |\ action::rest\ \Rightarrow\ \textbf{let}\ s'\ :=\ (step\ s\ action).st\ \textbf{in}\ s'::trace\ s'\ rest \\
	\quad \textbf{end.}
\end{array}
\end{displaymath}
\caption{The $trace$ function}
\label{fig:trace}
\end{figure}
We have also stated and proved security properties over the function $trace$, showing that the specification allows an implementation where they hold.

When the user grants the permission required for accessing a resource to an application, it may delegate such right to another one or even itself. Once the user revokes it, these delegations aren't invalidated and so the application may still be able to access the resource. This lemma is a proof that the current specification allows a behaviour which is arguably against the user's will.

\begin{lemma} [delegateGrantPRevoke] \label{impproperty1} \\
$	\forall 
	(s:\AndroidState)
	(p:\Perm)
	(app,app':\AppId)
	(ic,ic': \iComp)
	(c,c':\Comp)$ \\
$	(u:uri)
	(cp:CProvider), 
	valid\_state(s) \rightarrow 
	step(s,\texttt{grant}~p~app).resp = ok \rightarrow $ \\
$	getAppFromCmp(c,s) = app \rightarrow 
	getAppFromCmp(c',s) = app' \rightarrow$ \\
$	(ic, c) \in getRunningComponents(s) \rightarrow
	(ic', c') \in getRunningComponents(s) \rightarrow$ \\
$	canGrant(cp,u,s) \rightarrow 
existsRes(cp,u,s) \rightarrow 
componentIsExported(cp) \rightarrow$ \\
$	permissionRequiredForRead(cp) = Some~p \rightarrow$ \\
$	\mathsf{let}~opsResult := trace(s,\texttt{[}\texttt{grant}~p~app, \texttt{grantP}~ic~cp~app'~u~Read$,\\ 
$ \texttt{revoke}~p~app\texttt{]}~\mathsf{in}$ 
$	step(last(opsResult,s), \texttt{read}~ic'~cp~u).resp=ok$  \\ \\
\textit{In Android 6, revoking a permission doesn't invalidate the right of performing an operation over resources protected by it that the application may have delegated.}\\
\end{lemma}

The following property doesn't represent a security problem, but rather proves that a mildly complex requirement is met by the specification, providing theoretical background for it to be considered correct. \\

\begin{lemma}[ifPermThenGranted]\\
\label{impproperty2}
$	\forall
	(initState,lastState:\AndroidState)
	(app:AppId)
	(p:\Perm)
	(l: list\ \Action)$, \\
$	valid\_state(initState) \rightarrow 
	app \in getInstalledApps(initState) \rightarrow$ \\
$	getPermissionLevel(p)= dangerous \rightarrow 
	permissionIsGrouped(p) = None \rightarrow $ \\
$	appHasPermission(app,p,lastState) \rightarrow$\\
$	\neg appHasPermission(app,p,initState)\rightarrow
	\texttt{uninstall}~app \notin l \rightarrow $ \\
$	last(trace(initState,l),initState) = lastState \rightarrow 
	\texttt{grant}~p~app \in l$ \\ \\
\textit{In this operating system, the only way an application may have a non-grouped dangerous permission which it didn't have before, is by an explicit grant.}\\
\end{lemma}


Complementing Lemma~\ref{impproperty2}, the following lemma formally shows that a desired behaviour is in fact present in the system.

\begin{lemma}[revokeAndNotGrant]\\
$	\forall
	(initState,sndState,lastState:\AndroidState)
	(app:\AppId)
	(p:\Perm)
	(l: list~\Action)$, \\
$	valid\_state(initState) \rightarrow
	getPermissionLevel(p) = dangerous \rightarrow$ \\
$	permissionIsGrouped(p) = None \rightarrow
	p \notin getDefPermsForApp(app,initState) \rightarrow$ \\
$	step(initState,\texttt{revoke}~p~app).st = sndState \rightarrow$ \\
$	step(initState, \texttt{revoke}~p~app)).resp=ok \rightarrow$\\
$	\texttt{uninstall}~app \notin l \rightarrow
	\texttt{grant}~p~app \notin l \rightarrow $\\
$	last(trace(sndState,l),sndState) = lastState \rightarrow$\\
$	\neg appHasPermission(app,p,lastState)$ \\ \\
\textit{ If an application used to have a permission that was later revoked, only regranting it will allow the application to have it again.}\\
\end{lemma}

Certain assertions on which a developer could rely in previous versions of the operating system don't hold in its latest version. The following lemma is a formal example of one of them, and is useful to formally check that the new requirements cannot be bypassed and that old applications must be adapted to comply with the new requirements.
\begin{lemma}[revokeCanStart]\\
$	\forall
	(initState:\AndroidState)
%	(l: list \Action)
	(app,app': \AppId)
	(c:\Comp)
	(act:\Activity)
	(p:\Perm)$, \\
$	valid\_state(initState) \rightarrow 
	getPermissionLevel(p) = dangerous \rightarrow$ \\
$	permissionIsGrouped(p) = None \rightarrow 
	app \neq app' \rightarrow $\\
$	p \notin getDefPermsForApp(app,initState) \rightarrow 
	inApp(c,app,initState) \rightarrow$ \\
$	inApp(act,app',initState) \rightarrow 
	cmpProtectedByPerm(act) = Some~p \rightarrow$ \\
$	canStart(c,act,initState) \rightarrow 
	\exists (l: list\ \Action),
	\texttt{uninstall}~app \notin l\ \land$ \\
$	\texttt{uninstall}~app' \notin l \land
	\neg canStart(c,act,last(trace(initState,l), initState))$ \\ \\
\textit{	A running component may have the right of starting another one on a certain state, but may not be able to do so at a later time.}\\
\end{lemma}



==> run-time.tex <==
%\section{Requesting permissions at run time}
\section{Requesting (and granting) permissions at run time}
\label{sec:run-time}

On all versions of Android an application must declare both the normal and the dangerous permissions it needs in its application manifest. However, the effect of that declaration is different depending on the system version and the application's target SDK level \cite{android6}.
In particular, if a device is running Android 6.0 (Marshmallow) and the application's target SDK is 23 or higher
the application has to list the permissions in the manifest, and it must request each dangerous permission it needs while the application is running. The user can grant or deny each permission, and the application can continue to run with limited capabilities even if the user denies a permission request. This modification of the access control and decision process, on the one side, streamlines the application install process, since the user does not need to grant permissions when he/she installs or updates an application. On the other hand, as users can revoke the (previously granted) permissions at any time, the application needs to check whether it has the corresponding privileges every time it attempts to access a resource on the device.


\subsection{Impact on the formal model}
\label{sec:run-time-impact}
%On all versions of Android, an application need to declare both the normal and the dangerous permissions it needs in its application manifest. However, the effect of that declaration is different depending on the system version. % and the application's target SDK level \cite{android6}.
%In particular, if a device is running Android 6.0, %and the application's target SDK is 23 or higher: 
%the application has to list the permissions in the manifest, and it must request each dangerous permission it needs while the application is running. The user can grant or deny each permission, and the application can continue to run with limited capabilities even if the user denies a permission request.
%\end{itemize}

We have already modified the (formal) model presented and discussed in Section~\ref{sec:model} so as to consider the run time requesting/granting of permissions behavior introduced in Android Marshmallow. We shall not describe in detail the changes that were carried out and shall limit ourselves to provide some hints concerning the impact the changes had on the essential components of the model:  

\begin{itemize}
\item The application definition, as depicted in Figure~\ref{fig:model:application}, has not changed. In particular, the \texttt{AndroidManifest} remains the same 
%\footnote{On all versions of Android, an application need to declare both the normal and the dangerous permissions it needs in its application manifest. However, the effect of that declaration is different depending on the system version.}. 
\item The state (of type $\AndroidState$) remains unchanged. Also, the validity conditions of state (\textit{validState}) remain invariant.
\item Action $\mathtt{install}$ is simplified; the controls associated with dangerous permissions are removed.  
\item We have already incorporated actions to model the granting and revocation of a permission at run time.
\item The properties formalized in Section~\ref{sec:properties} remain valid. 
\end{itemize}

\subsection{On the security policies}
\label{sec:run-time-observations}

In this section we briefly discuss how the management of permissions has been affected by the design changes introduced in Android Marshmallow.

%\begin{itemize}
%\item \textit{Delegated permissions:} 
\paragraph*{Delegated permissions}
The official Android documentation does not specify what should happen when permissions acquired and delegated at run time by an application are revoked by the user. The delegation of a permission on a given resource might grant an application access to sensitive information that otherwise it would not have had. A (malicious) application could gain a permission for access sensitive data indefinitely in the case an user revokes a permission and not all delegations and re-delegations of this permission are also revoked.

%\item \textit{Permission groups:} 
\paragraph*{Permission groups}
A significant change in the new version of Android is that all dangerous system permissions belong to permission groups.  For example, if an application requires permission to read contacts, it must request access to the group \textit{android.permission-group.CONTACTS} that allows the application to read contacts, but also write and access the user's profile. 
% \gusnote{No me queda claro el escenario a continuacion} \cnote{Puse una nota al pie; la observación original fue planteada por Camila}
The biggest drawback with this change is that individual permissions remain. Applications developed in the latest version of Android could start applications developed in previous versions, using the individual permissions that, in principle, should not have\footnote{Individual permissions obtained (indirectly) from a permission group.}.
This behavior can induce \textit{privilege escalation} and also shows a lack of transparency with the user, who should accept that their applications have permissions to perform operations available on your sensitive data.

%\item \textit{Automatic Internet access:} 
\paragraph*{Automatic Internet access}
Another significant change is that permission to access the Internet becomes normal type. This means that all applications can potentially access the Internet without that permission being granted by the user of the device. For example, a flashlight application can access the Internet and the user can not do anything about it.
Android developers justify this change by saying that users are still the ones who grant permissions to access sensitive data. However, applications which by their nature can manipulate sensitive data have now also automatically access to the Internet. For example until Android Lollipop, a camera application which had granted access to images but was denied access to the web could be considered a safe application.
Users whose devices run Android Marshmallow have no means to know, for instance, if the camera has Internet access, so these applications would potentially no longer be safe.

%\item \textit{Missing permissions:} 
\paragraph*{Missing permissions}
Android Marshmallow allows users to revoke permissions from any application at any time. A developer should test his application to verify that it behaves properly when it is missing a needed permission. In particular, the user can grant or deny each dangerous permission, and the application can continue to run with limited capabilities even after a user has denied a permission request.

%\item \textit{Social engineering:} 
\paragraph*{Social engineering attacks}
The request of dangerous run time permissions might give rise to the generation of new patterns of attacks based on social engineering. A detailed analysis in this direction has already been identified as future work.
%\end{itemize}

%\cnote{explicar cambio en la v.6 respecto a permisos en tiempo de ejecución, discutir impacto en el modelo (no cambia el estado pero se agrgan dos acciones) y hacer un analisis conceptual de la extension, destacando posibles problemas.}


%Android Marshmallow (version 6.0) introduces a new spin on application permissions in an attempt to simplify permissions and to reduce the number of permissions needed.
%Beginning in Android 6.0, users grant dangerous permissions to applications while the application is running, not when they install the application. This approach streamlines the application install process, since the user does not need to grant permissions when they install or update the application. Also, the user can revoke the permissions at any time, so the application needs to check whether it has the permissions every time it runs \cite{android6}.
%
%
%\subsection{Impact on the formal model}
%\label{sec:run-time-impact}
%%On all versions of Android, an application need to declare both the normal and the dangerous permissions it needs in its application manifest. However, the effect of that declaration is different depending on the system version. % and the application's target SDK level \cite{android6}.
%%In particular, if a device is running Android 6.0, %and the application's target SDK is 23 or higher: 
%%the application has to list the permissions in the manifest, and it must request each dangerous permission it needs while the application is running. The user can grant or deny each permission, and the application can continue to run with limited capabilities even if the user denies a permission request.
%%\end{itemize}
%
%
%The (formal) model specified in Section~\ref{sec:model}
%essentially contemplates the changes introduced by the latest version of Android. Below we describe some relevant considerations:
%\begin{itemize}
%\item The application definition, as depicted in Figure~\ref{fig:model:application}, is not changed. In particular, the \texttt{AndroidManifest} is the same\footnote{On all versions of Android, an application need to declare both the normal and the dangerous permissions it needs in its application manifest. However, the effect of that declaration is different depending on the system version.}. 
%\item The state (of type $\AndroidState$) remains unchanged. Also, the validity conditions of state (\textit{validState}) remain invariant.
%\item Action $\mathtt{install}$ is simplified; the controls associated with dangerous permissions are removed.  
%\item Actions are incorporated to model the granting and revocation of a permission at run time.
%\item The properties formalized in Section~\ref{sec:properties} remain valid. 
%\end{itemize}
%
%\subsection{Observations}
%\label{sec:run-time-observations}
%
%In this section we discuss some consequences introduced by the latest version of Android that relate to the management of permissions.
%
%%\begin{itemize}
%%\item \textit{Delegated permissions:} 
%\paragraph*{Delegated permissions}
%The official Android documentation does not specify what should happen if an application delegate permissions obtained at run time, which will then be revoked.
%In this case, an application might acquire permissions that were never requested to the user permanently.
%Beyond the lack of transparency with the user, which is one of the main objectives of the latest version of Android, a problem is generated in system security.
%By delegating permissions on a resource to an application is allowed access to sensitive information that otherwise would not have. A malicious application could be gaining permissions for access sensitive data indefinitely if when the user revokes a permission, not all delegations and re-delegations of this permission is also revoked.
%
%%\item \textit{Permission groups:} 
%\paragraph*{Permission groups}
%From Android Marshmallow, all dangerous system permissions belong to permission groups. 
%For example, if an application requires permission to read contacts, it must request access to the group \textit{android.permission-group.CONTACTS} that allows the application to read contacts, but also write and access the user's profile.
%The biggest drawback with this change is that individual permissions remain. Applications developed in the latest version of Android could start applications developed in previous versions, using the individual permissions that, in principle, should not have.
%This behavior can induce \textit{privilege escalation} and also shows a lack of transparency with the user, who should accept that their applications have permissions to perform operations available on your sensitive data.
%
%%\item \textit{Automatic Internet access:} 
%\paragraph*{Automatic Internet access}
%A significant change in the new version of Android is that permission to access the Internet becomes normal type. This means that all applications can access the Internet without the user can grant or revoke this permission. For example, a flashlight application can access the Internet and the user can not do anything about it.
%Android developers justify this change by saying that users are those who decide to grant permission to access sensitive data, but those applications which by their nature can manipulate sensitive data have now also automatically access to the Internet.
%For example until Android Lollipop, the camera with access to images but without access to the web was considered a safe application.
%Beginning in Android Marshmallow, users can not know if the camera has Internet access, so these applications would no longer be safe.
%
%
%%\item \textit{Missing permissions:} 
%\paragraph*{Missing permissions}
%Beginning with Android 6.0, users can revoke permissions from any application at any time. A developer should test your application to verify that it behaves properly when it's missing a needed permission. In particular, the user can grant or deny each dangerous permission, and the application can continue to run with limited capabilities even if the user denies a permission request.
%
%%\item \textit{Social engineering:} 
%\paragraph*{Social engineering attacks}
%Request dangerous run time permissions could influence the generation of new patterns of attacks based on social engineering. A detailed analysis in this direction is proposed as future work.
%%\end{itemize}
%
%%\cnote{explicar cambio en la v.6 respecto a permisos en tiempo de ejecución, discutir impacto en el modelo (no cambia el estado pero se agrgan dos acciones) y hacer un analisis conceptual de la extension, destacando posibles problemas.}


==> semgrantT.tex <==
%\small
%\begin{figure}[b]
\actdefsection{Action \action{grantT} $ic$ $cp$ $act$ $u$ $pt$}
%Description

\begin{actdef}{The running component $ic$ delegates temporary permissions to activity $act$. This delegation enables $act$ to perform operation $pt$ on the resource assigned to URI $u$ from content provider $cp$.}
%Rule  

\begin{actdefrule}
\inferrule
{\bap{\mathit{compInstalled}}{cp}{s} \land 
\tap{\mathit{canGrant}}{u}{cp}{s} \land 
\tap{\mathit{existsRes}}{u}{cp}{s}\ \land \\
\bap{\mathit{compInstalled}}{act}{s} \land
\exists(c:Comp), \bap{\mathit{compInstalled}}{c}{s}\ \land \\ 
\tap{\mathit{running}}{ic}{c}{s} \land 
\tap{\mathit{canStart}}{act}{c}{s}\ \land \\ 
(\qap{\mathit{canOp}}{c}{cp}{pt}{s} \lor \fap{\mathit{delPerms}}{c}{cp}{u}{pt}{s})\ \land \\ 
s=(aps, ps, psD, iCs, delPP, delTP, v, img)  \\
\exists~(ic':iComp),\bap{\mathit{insNotInState}}{ic'}{s} \land ~~~~~~~~~~~~ \\
\tap{\mathit{runComp}}{ic'}{act}{s}=iCs' \land
\fap{\mathit{grantTPerm}}{ic'}{cp}{u}{pt}{s}=delTP'\ \land \\ s'=(aps, ps, psD, iCs', delPP, delTP', v, img) 
}
{s \semstep{\agrantt{ic}{cp}{act}{u}{pt}} s'} %\\[5ex]
\end{actdefrule}

\vspace{4pt} 
\noindent
\textbf{Precondition~}
The content provider $cp$ is installed in state $s$.
Permissions can be delegated on $cp$ for resource identified by the URI $u$. 
The component $act$ is an activity installed in $s$.
The component $ic$ is a running instance of a component ($c$) that belongs to an installed application in $s$.
The application containing component $act$ has the required permissions to create a new running instance of component $c$. 
Additionally, the application containing component $c$ either has the appropriate permissions to perform the operation $pt$ on $cp$ or it has has been delegated permissions to perform $pt$ on the resource identified by $u$. \\
%
\textbf{Postcondition~} 
A new running component instance of activity $act$ is incorporated into the system state. Moreover, a new temporary delegated permission corresponding to the running instance generated is added into the temporary permissions delegations of state $s$. This delegation enables $act$ to perform $pt$ on the resource assigned to $u$ from $cp$.
Apart from that, both states are equal.

\end{actdef}
